Standardised formats and open-source analysis tools for the MAGIC telescopes data

Instruments for gamma-ray astronomy at Very High Energies ($E>100\,{\rm GeV}$) have traditionally derived their scientific results through proprietary data and software. Data standardisation has become a prominent issue in this field both as a requirement for the dissemination of data from the next generation of gamma-ray observatories and as an effective solution to realise public data legacies of current-generation instruments. Specifications for a standardised gamma-ray data format have been proposed as a community effort and have already been successfully adopted by several instruments. We present the first production of standardised data from the Major Atmospheric Gamma-ray Imaging Cherenkov (MAGIC) telescopes. We converted $166\,{\rm h}$ of observations from different sources and validated their analysis with the open-source software Gammapy. We consider six data sets representing different scientific and technical analysis cases and compare the results obtained analysing the standardised data with open-source software against those produced with the MAGIC proprietary data and software. Aiming at a systematic production of MAGIC data in this standardised format, we also present the implementation of a database-driven pipeline automatically performing the MAGIC data reduction from the calibrated down to the standardised data level. In all the cases selected for the validation, we obtain results compatible with the MAGIC proprietary software, both for the manual and for the automatic data productions. Part of the validation data set is also made publicly available, thus representing the first large public release of MAGIC data. This effort and this first data release represent a technical milestone toward the realisation of a public MAGIC data legacy.

==> opted-in_associated_2202_2024-01-02.tex <==
% authors 2024-01-02, poll ID 2202, Format elsartJheap
%
\author[1]{K.~Ishio}  -  ishio@mpp.mpg.de
\author[2]{D.~Morcuende}  -  dmorcuende@iaa.es
\author[3]{K.~Noda}  -  nodak@icrr.u-tokyo.ac.jp
\author[2]{J.~Otero-Santos}  -  joteros@iaa.es
\address[1]{University of Lodz, Faculty of Physics and Applied Informatics, Department of Astrophysics, 90-236 Lodz, Poland}
\address[2]{Instituto de Astrof\'isica de Andaluc\'ia-CSIC, Glorieta de la Astronom\'ia s/n, 18008, Granada, Spain}
\address[3]{Japanese MAGIC Group: Chiba University, ICEHAP, 263-8522 Chiba, Japan}


==> opted-in_collaborators_2202_2024-01-02.tex <==
% authors 2024-01-02, poll ID 2202, Format elsartJheap
%
\author[1]{S.~Abe}
\author[2]{J.~Abhir}
\author[3]{A.~Abhishek}
\author[4]{V.~A.~Acciari}
\author[5]{A.~Aguasca-Cabot}
\author[6]{I.~Agudo}
\author[7]{T.~Aniello}
\author[8,41]{S.~Ansoldi}
\author[7]{L.~A.~Antonelli}
\author[9]{A.~Arbet Engels}
\author[10]{C.~Arcaro}
\author[4]{M.~Artero}
\author[1]{K.~Asano}
\author[11]{A.~Babi\'c}
\author[12]{U.~Barres de Almeida}
\author[13]{J.~A.~Barrio}
\author[10]{I.~Batkovi\'c}
\author[9]{A.~Bautista}
\author[1]{J.~Baxter}
\author[14]{J.~Becerra Gonz\'alez}
\author[15]{W.~Bednarek}
\author[10]{E.~Bernardini}
\author[16]{J.~Bernete}
\author[9]{A.~Berti}
\author[9]{J.~Besenrieder}
\author[7]{C.~Bigongiari}
\author[2]{A.~Biland}
\author[4]{O.~Blanch}
\author[7]{G.~Bonnoli}
\author[11]{\v{Z}.~Bo\v{s}njak}
\author[7]{E.~Bronzini}
\author[8]{I.~Burelli}
\author[10]{G.~Busetto}
\author[17]{A.~Campoy-Ordaz}
\author[7]{A.~Carosi}
\author[18]{R.~Carosi}
\author[5]{M.~Carretero-Castrillo}
\author[6]{A.~J.~Castro-Tirado}
\author[19]{D.~Cerasole}
\author[9]{G.~Ceribella}
\author[1]{Y.~Chai}
\author[16]{A.~Cifuentes}
\author[4]{E.~Colombo}
\author[13]{J.~L.~Contreras}
\author[16]{J.~Cortina}
\author[7]{S.~Covino}
\author[20]{G.~D'Amico}
\author[7]{V.~D'Elia}
\author[7]{P.~Da Vela}
\author[7]{F.~Dazzi}
\author[10]{A.~De Angelis}
\author[8]{B.~De Lotto}
\author[21]{R.~de Menezes}
\author[4,42]{M.~Delfino}
\author[4,42]{J.~Delgado}
\author[21]{F.~Di Pierro}
\author[19]{R.~Di Tria}
\author[19]{L.~Di Venere}
\author[22]{D.~Dominis Prester}
\author[7]{A.~Donini}
\author[23]{D.~Dorner}
\author[10]{M.~Doro}
\author[24]{D.~Elsaesser}
\author[6]{J.~Escudero}
\author[4]{L.~Fari\~na}
\author[24]{A.~Fattorini}
\author[7]{L.~Foffano}
\author[17]{L.~Font}
\author[24]{S.~Fr\"ose}
\author[2]{S.~Fukami}
\author[25]{Y.~Fukazawa}
\author[14]{R.~J.~Garc\'ia L\'opez}
\author[26]{M.~Garczarczyk}
\author[27]{S.~Gasparyan}
\author[17]{M.~Gaug}
\author[12]{J.~G.~Giesbrecht Paiva}
\author[19]{N.~Giglietto}
\author[19]{F.~Giordano}
\author[15]{P.~Gliwny}
\author[24]{T.~Gradetzke}
\author[4]{R.~Grau}
\author[9]{D.~Green}
\author[9]{J.~G.~Green}
\author[23]{P.~G\"unther}
\author[1]{D.~Hadasch}
\author[9]{A.~Hahn}
\author[16]{T.~Hassan}
\author[9]{L.~Heckmann}
\author[14]{J.~Herrera Llorente}
\author[28]{D.~Hrupec}
\author[1]{M.~H\"utten}
\author[25]{R.~Imazawa}
\author[15]{K.~Ishio}
\author[9]{I.~Jim\'enez Mart\'inez}
\author[29]{J.~Jormanainen}
\author[25]{T.~Kayanoki}
\author[4]{D.~Kerszberg}
\author[20,43]{G.~W.~Kluge}
\author[1]{Y.~Kobayashi}
\author[29]{P.~M.~Kouch}
\author[1]{H.~Kubo}
\author[30]{J.~Kushida}
\author[13]{M.~L\'ainez}
\author[7]{A.~Lamastra}
\author[7]{F.~Leone}
\author[29]{E.~Lindfors}
\author[7]{S.~Lombardi}
\author[8,44]{F.~Longo}
\author[6]{R.~L\'opez-Coto}
\author[13]{M.~L\'opez-Moya}
\author[14]{A.~L\'opez-Oramas}
\author[19]{S.~Loporchio}
\author[3]{A.~Lorini}
\author[31]{E.~Lyard}
\author[12]{B.~Machado de Oliveira Fraga}
\author[32]{P.~Majumdar}
\author[33]{M.~Makariev}
\author[33]{G.~Maneva}
\author[22]{M.~Manganaro}
\author[16]{S.~Mangano}
\author[23]{K.~Mannheim}
\author[10]{M.~Mariotti}
\author[4]{M.~Mart\'inez}
\author[16]{M.~Mart\'inez-Chicharro}
\author[13]{A.~Mas-Aguilar}
\author[1,45]{D.~Mazin}
\author[6]{S.~Menchiari}
\author[24]{S.~Mender}
\author[10]{D.~Miceli}
\author[13]{T.~Miener}
\author[3]{J.~M.~Miranda}
\author[9]{R.~Mirzoyan}
\author[14]{M.~Molero Gonz\'alez}
\author[14]{E.~Molina}
\author[32]{H.~A.~Mondal}
\author[4]{A.~Moralejo}
\author[6]{D.~Morcuende}
\author[34]{T.~Nakamori}
\author[7]{C.~Nanci}
\author[35]{V.~Neustroev}
\author[24]{L.~Nickel}
\author[14]{M.~Nievas Rosillo}
\author[4]{C.~Nigro}
\author[3]{L.~Nikoli\'c}
\author[30]{K.~Nishijima}
\author[4]{T.~Njoh Ekoume}
\author[36]{K.~Noda}
\author[9]{S.~Nozaki}
\author[1]{Y.~Ohtani}
\author[37]{A.~Okumura}
\author[6]{J.~Otero-Santos}
\author[7]{S.~Paiano}
\author[9]{D.~Paneque}
\author[3]{R.~Paoletti}
\author[5]{J.~M.~Paredes}
\author[9]{M.~Peresano}
\author[8,46]{M.~Persic}
\author[10]{M.~Pihet}
\author[9]{G.~Pirola}
\author[3]{F.~Podobnik}
\author[18]{P.~G.~Prada Moroni}
\author[10]{E.~Prandini}
\author[8]{G.~Principe}
\author[4]{C.~Priyadarshi}
\author[24]{W.~Rhode}
\author[5]{M.~Rib\'o}
\author[4]{J.~Rico}
\author[7]{C.~Righi}
\author[27]{N.~Sahakyan}
\author[1]{T.~Saito}
\author[7]{F.~G.~Saturni}
\author[24]{K.~Schmidt}
\author[9]{F.~Schmuckermaier}
\author[24]{J.~L.~Schubert}
\author[9]{T.~Schweizer}
\author[7]{A.~Sciaccaluga}
\author[10]{G.~Silvestri}
\author[15]{J.~Sitarek}
\author[31]{V.~Sliusar}
\author[15]{D.~Sobczynska}
\author[10]{A.~Spolon}
\author[7]{A.~Stamerra}
\author[28]{J.~Stri\v{s}kovi\'c}
\author[9]{D.~Strom}
\author[1]{M.~Strzys}
\author[25]{Y.~Suda}
\author[29]{S.~Suutarinen}
\author[37]{H.~Tajima}
\author[37]{M.~Takahashi}
\author[1]{R.~Takeishi}
\author[33]{P.~Temnikov}
\author[38]{K.~Terauchi}
\author[22]{T.~Terzi\'c}
\author[9,47]{M.~Teshima}
\author[3]{S.~Truzzi}
\author[7]{A.~Tutone}
\author[17]{S.~Ubach}
\author[9]{J.~van Scherpenberg}
\author[14]{M.~Vazquez Acosta}
\author[3]{S.~Ventura}
\author[10]{I.~Viale}
\author[21]{C.~F.~Vigorito}
\author[39]{V.~Vitale}
\author[1]{I.~Vovk}
\author[31]{R.~Walter}
\author[9]{M.~Will}
\author[3]{C.~Wunderlich}
\author[40]{T.~Yamamoto}
\address[1]{Japanese MAGIC Group: Institute for Cosmic Ray Research (ICRR), The University of Tokyo, Kashiwa, 277-8582 Chiba, Japan}
\address[2]{ETH Z\"urich, CH-8093 Z\"urich, Switzerland}
\address[3]{Universit\`a di Siena and INFN Pisa, I-53100 Siena, Italy}
\address[4]{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}
\address[5]{Universitat de Barcelona, ICCUB, IEEC-UB, E-08028 Barcelona, Spain}
\address[6]{Instituto de Astrof\'isica de Andaluc\'ia-CSIC, Glorieta de la Astronom\'ia s/n, 18008, Granada, Spain}
\address[7]{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}
\address[8]{Universit\`a di Udine and INFN Trieste, I-33100 Udine, Italy}
\address[9]{Max-Planck-Institut f\"ur Physik, D-85748 Garching, Germany}
\address[10]{Universit\`a di Padova and INFN, I-35131 Padova, Italy}
\address[11]{Croatian MAGIC Group: University of Zagreb, Faculty of Electrical Engineering and Computing (FER), 10000 Zagreb, Croatia}
\address[12]{Centro Brasileiro de Pesquisas F\'isicas (CBPF), 22290-180 URCA, Rio de Janeiro (RJ), Brazil}
\address[13]{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}
\address[14]{Instituto de Astrof\'isica de Canarias and Dpto. de  Astrof\'isica, Universidad de La Laguna, E-38200, La Laguna, Tenerife, Spain}
\address[15]{University of Lodz, Faculty of Physics and Applied Informatics, Department of Astrophysics, 90-236 Lodz, Poland}
\address[16]{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas, E-28040 Madrid, Spain}
\address[17]{Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain}
\address[18]{Universit\`a di Pisa and INFN Pisa, I-56126 Pisa, Italy}
\address[19]{INFN MAGIC Group: INFN Sezione di Bari and Dipartimento Interateneo di Fisica dell'Universit\`a e del Politecnico di Bari, I-70125 Bari, Italy}
\address[20]{Department for Physics and Technology, University of Bergen, Norway}
\address[21]{INFN MAGIC Group: INFN Sezione di Torino and Universit\`a degli Studi di Torino, I-10125 Torino, Italy}
\address[22]{Croatian MAGIC Group: University of Rijeka, Faculty of Physics, 51000 Rijeka, Croatia}
\address[23]{Universit\"at W\"urzburg, D-97074 W\"urzburg, Germany}
\address[24]{Technische Universit\"at Dortmund, D-44221 Dortmund, Germany}
\address[25]{Japanese MAGIC Group: Physics Program, Graduate School of Advanced Science and Engineering, Hiroshima University, 739-8526 Hiroshima, Japan}
\address[26]{Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany}
\address[27]{Armenian MAGIC Group: ICRANet-Armenia, 0019 Yerevan, Armenia}
\address[28]{Croatian MAGIC Group: Josip Juraj Strossmayer University of Osijek, Department of Physics, 31000 Osijek, Croatia}
\address[29]{Finnish MAGIC Group: Finnish Centre for Astronomy with ESO, Department of Physics and Astronomy, University of Turku, FI-20014 Turku, Finland}
\address[30]{Japanese MAGIC Group: Department of Physics, Tokai University, Hiratsuka, 259-1292 Kanagawa, Japan}
\address[31]{University of Geneva, Chemin d'Ecogia 16, CH-1290 Versoix, Switzerland}
\address[32]{Saha Institute of Nuclear Physics, A CI of Homi Bhabha National Institute, Kolkata 700064, West Bengal, India}
\address[33]{Inst. for Nucl. Research and Nucl. Energy, Bulgarian Academy of Sciences, BG-1784 Sofia, Bulgaria}
\address[34]{Japanese MAGIC Group: Department of Physics, Yamagata University, Yamagata 990-8560, Japan}
\address[35]{Finnish MAGIC Group: Space Physics and Astronomy Research Unit, University of Oulu, FI-90014 Oulu, Finland}
\address[36]{Japanese MAGIC Group: Chiba University, ICEHAP, 263-8522 Chiba, Japan}
\address[37]{Japanese MAGIC Group: Institute for Space-Earth Environmental Research and Kobayashi-Maskawa Institute for the Origin of Particles and the Universe, Nagoya University, 464-6801 Nagoya, Japan}
\address[38]{Japanese MAGIC Group: Department of Physics, Kyoto University, 606-8502 Kyoto, Japan}
\address[39]{INFN MAGIC Group: INFN Roma Tor Vergata, I-00133 Roma, Italy}
\address[40]{Japanese MAGIC Group: Department of Physics, Konan University, Kobe, Hyogo 658-8501, Japan}
\address[41]{also at International Center for Relativistic Astrophysics (ICRA), Rome, Italy}
\address[42]{also at Port d'Informaci\'o Cient\'ifica (PIC), E-08193 Bellaterra (Barcelona), Spain}
\address[43]{also at Department of Physics, University of Oslo, Norway}
\address[44]{also at Dipartimento di Fisica, Universit\`a di Trieste, I-34127 Trieste, Italy}
\address[45]{Max-Planck-Institut f\"ur Physik, D-85748 Garching, Germany}
\address[46]{also at INAF Padova}
\address[47]{Japanese MAGIC Group: Institute for Cosmic Ray Research (ICRR), The University of Tokyo, Kashiwa, 277-8582 Chiba, Japan}

